TALM: Tool Augmented Language Models

Transformer based language models (LMs) demonstrate increasing performance with scale across a wide variety of tasks. Scale alone however cannot enable models to solve tasks that require access to ephemeral, changing, or private data that was unavailable at training time. Many useful tasks may also benefit from LMs being able to access APIs that read or modify state. In this work, we present Tool Augmented Language Models (TALM), combining a text-only approach to augment language models with non-differentiable tools, and an iterative "self-play" technique to bootstrap performance starting from few tool demonstrations. TALM exhibits strong performance on both a knowledge-heavy QA task and a reasoning oriented math task with simple tools. At a given model scale, TALM significantly outperforms non-augmented LMs. We further demonstrate that TALM successfully performs out-of-distribution inferences on both QA and math tasks, where non-augmented LMs fail. Our results suggest that Tool Augmented Language Models are a promising direction to enrich LMs' capabilities, with less dependence on scale.

==> figures/nq_self_play_flow.tex <==

\begin{figure}[tbh]
\centering
\includegraphics[width=0.45\textwidth]{figures/NQSelfPlayFlowchart.png}
\caption{some text}
\label{fig:filter}
\end{figure}


==> figures/ood_chain.tex <==
% originally h! - try ht or htbp
\begin{figure}[H]
\centering

\begin{mdframed}
\small

\textbf{Question:}
\textcolor{teal}{ What is the total number of parameters in Gopher, Chinchilla and GPT-3 in B?} 
\vspace{3pt}

\textbf{Search Tool Input:}
\textcolor{orange}{Gopher, Chinchilla and GPT-3} 
\vspace{3pt}

\textbf{Search Tool Output:}
\textcolor{blue}{"Researchers found that Chinchilla \u201cuniformly and significantly\u201d outperforms Gopher, GPT-3, Jurassic-1, and Megatron-Turing NLG across a large set of language\u00a0.  Check Out This DeepMind's New Language Model, Chinchilla (70B Parameters), Which Significantly Outperforms Gopher (280B) and GPT-3 (175B) on ...} 

\textbf{Math Tool Input:}
\textcolor{orange}{add ( add ( 280 , 175 ) , 70 )} 
\vspace{3pt}

\textbf{Math Tool Output:}
\textcolor{violet}{525} 
% colors: orange, blue, violet, teal

\end{mdframed}
\vspace{-5pt}

\caption{LM vs TALM on large number operation.}
\label{fig:ood_math}
\end{figure}



==> figures/tool_use_example2.tex <==
\begin{figure}[h!]
\centering
% \includegraphics[width=1.0\linewidth]{figures/tool_use_sequence_v03.pdf}
%\caption{Comparison of traditional and tool augmented language models.}
%\caption{Tool Augmented Language Models can access arbitrary tools via a text to text API.}
% \caption{Traditional and Tool Augmented LMs.}

\begin{mdframed}
\small

\textbf{Subtask 1 (call tool)}

\textcolor{teal}{task input text} $\Rightarrow$ \textcolor{orange}{\emph{\textbf{\textbar tool-call}} tool input text}
\vspace{3pt}


\textbf{Subtask 2 (generate answer)}

\textcolor{teal}{task input text} 
\textcolor{orange}{\emph{\textbf{\textbar tool-call}} tool input text} 
\textcolor{blue}{\emph{\textbf{\textbar result}} tool output text} 
$\Rightarrow$ \textcolor{violet}{\emph{\textbf{\textbar output}} task output text} 


\iffalse
\textbf{Task 3 (decoder-only alternate)}

\textcolor{teal}{task input text} 
\textcolor{orange}{tool-call\textbar tool input text} 
\textcolor{blue}{result\textbar to output text} 
\textcolor{violet}{answer\textbar task output text} 
\fi


\end{mdframed}
\vspace{-10pt}
% \caption{Tool Augmented Language Model.}
\caption{TALM training subtasks.}
\label{fig:tasks_example}
\end{figure}

==> figures/unused_tool_use_example.tex <==
\begin{figure}[h!]
\centering

\begin{mdframed}
\small

\textbf{Task 1}

\textcolor{teal}{[input]: task input text} $\Rightarrow$ \textcolor{orange}{\textbf{[tool input]:} tool input text}
\vspace{3pt}

\textbf{Task 2}

\textcolor{teal}{[input]: task input text} 
\textcolor{orange}{[tool input]: tool input text} 
\textcolor{blue}{[tool output]: task output text} 
$\Rightarrow$ \textcolor{violet}{[result]: task output text} 

\end{mdframed}

\caption{Tool augmented language model training tasks}
\label{fig:tasks_example}
\end{figure}
